Dandelion++: Lightweight Cryptocurrency Networking with Formal Anonymity Guarantees

Recent work has demonstrated significant anonymity vulnerabilities in Bitcoin's networking stack. In particular, the current mechanism for broadcasting Bitcoin transactions allows third-party observers to link transactions to the IP addresses that originated them. This lays the groundwork for low-cost, large-scale deanonymization attacks. In this work, we present Dandelion++, a first-principles defense against large-scale deanonymization attacks with near-optimal information-theoretic guarantees. Dandelion++ builds upon a recent proposal called Dandelion that exhibited similar goals. However, in this paper, we highlight simplifying assumptions made in Dandelion, and show how they can lead to serious deanonymization attacks when violated. In contrast, Dandelion++ defends against stronger adversaries that are allowed to disobey protocol. Dandelion++ is lightweight, scalable, and completely interoperable with the existing Bitcoin network. We evaluate it through experiments on Bitcoin's mainnet (i.e., the live Bitcoin network) to demonstrate its interoperability and low broadcast latency overhead.

==> attack.tex <==
\subsection{\red{Attack (Remove this section?)}}
\label{sec:attack}

Although several papers have presented anonymity attacks on Bitcoin's flooding protocol, prior attacks have not exploited an important attack vector:
most Bitcoin implementations allow nodes to check whether a given peer has already seen a particular transaction.
To understand this capability, we start with a more detailed explanation of how content gets propagated.

Suppose a node (Alice) comes to possess a new transaction \texttt{tx} (either by creating the transaction or by receiving it from a peer).
Alice first runs basic validity checks on \texttt{tx} (e.g., is it signed properly? does the transaction draw funds from a known valid transaction output?).
If \texttt{tx} passes these checks, Alice adds it to a local memory store of recent transactions called the \texttt{mempool}.
If \texttt{tx}  depends on an earlier transaction that is yet unseen (e.g., due to randomness in network propagation), \texttt{tx} is added to the \emph{orphan cache}, 
a data structure containing so-called \emph{orphan transactions}.
\texttt{tx} remains in the orphan cache until either a valid parent transaction is received, or the transaction expires and gets flushed from the cache.

If \texttt{tx} is a valid transaction, instead of relaying \texttt{tx} to her neighbors, Alice first sends an inventory (\texttt{INV}) message containing the transaction hash to each of her neighbors. 
%This is intended to reduce communication costs in the network.
Upon receiving an \texttt{INV}, each peer node (Bob) checks its local \texttt{mempool} to see if it has previously received the transaction.
If so, Bob does nothing.
If not, Bob responds with a \texttt{GETDATA} message, which requests the full transaction;
at this point, Alice sends the full transaction. 

Notice that these two data structures---\texttt{mempool} and the orphan cache---collectively contain a history of which transactions have been recently seen by a given node. 
There are several ways that an adversary could probe these data structures to check if a given transaction has been seen by a target node.
First, consider a transaction in the \texttt{mempool}.
An adversary could send a spurious \texttt{GETDATA} message to the target requesting a given transaction \texttt{tx};
if that transaction is in the target's \texttt{mempool}, he will respond with \texttt{tx}.
%Hence, if an adversary wanted to test if a given transaction has been seen by a particular node, acces
Moreover, in 2012, Bitcoin Core added a `mempool' P2P command, which causes the recipient to respond with the full contents of her \texttt{mempool}.
Now suppose the transaction is still in the orphan cache. 

\subsection{Summary}
%Among the proposed solutions in this space, we contend that \Algo~ is the closest to a workable one: it is lightweight, distributed, and Bitcoin-compatible, while still providing some degree of provable, population-wide anonymity guarantees.
In this paper, we propose a lightweight, provably-anonymous flooding policy that uses \Algo~ as a starting point.
As discussed previously, \Algo~is far from practical in its current state.
First and foremost, it is unclear if and how its anonymity guarantees extend to realistic attack scenarios with Byzantine nodes, partial deployment, etc.
Indeed, we show that \Algo's anonymity guarantees are fragile to active attackers.
Second, \cite{dand} did not actually evaluate the practical latency and/or implementation overhead of \Algo.
In this paper, we address these weaknesses by proposing a revised policy, \Algopp, that provides stronger robustness and anonymity properties, both in theory and in practice.
We also implement \Algopp~and test it in the Bitcoin network to demonstrate that it incurs minimal latency overhead compared to the status quo of diffusion-based broadcasting. 
We begin by presenting a practical, lightweight attack and demonstrating its impact on the privacy guarantees of both diffusion and \Algo.  %adversarial model and problem formulation.



==> baselines.tex <==
\section{Motivation and Context}
\label{sec:context}

%The Bitcoin P2P network has received increasing attention in recent years. 
The cryptocurrency community has become increasingly aware of vulnerabilities in the P2P network.
This section gives an overview of P2P-network-based deanonymization attacks, suggested countermeasures, and their respective pros and cons.
We begin by introducing the broadcast mechanism underlying Bitcoin's P2P vulnerabilities, 
and then argue that proposed solutions in this space have been too ad-hoc, complex, or  naive to provide significant practical benefits.

\subsection{Trickle spreading}
When the Bitcoin reference implementation was first released, it used a broadcasting protocol called \emph{trickle spreading} \cite{bitcoindTrickleDiffusion}. 
Trickle spreading is a gossip protocol, in which each node transmits transactions to exactly one randomly-selected neighbor at a time.
The precise mechanism of trickle spreading is not important to our work; 
the point is that it---and its associated implementation---exhibited several weaknesses, including the fact that an attacker could cause a node to abandon trickle spreading altogether in favor of instantaneous flooding.

In 2014, researchers used trickle spreading to link transactions to the IP addresses that originated them \cite{biryukov,miers2013zerocoin,koshy2014analysis}. 
These attacks proceeded by connecting a supernode to a majority of active Bitcoin server nodes.
Regular nodes were unable to distinguish the supernode from other nodes, and therefore relayed content to it according to the usual trickle protocol.
For each transaction, the supernode would record the timestamps at which regular nodes relayed the transaction to the supernode.
Given these observations, a variant of the simple-yet-robust \emph{first-spy estimator} was used to link the measurements to an IP address.
The first-spy estimator outputs the first IP address to deliver a given transaction to the supernode as the estimated source.
Using this technique, the authors were able to link transactions to source IP addresses up to 30\% of the time, in both client and server nodes \cite{koshy2014analysis,biryukov}. 


\subsection{Proposed solutions}
In response to these attacks, the Bitcoin community proposed a number of candidate solutions. 
For example, the original attack papers proposed various heuristics aimed at mitigating the demonstrated attacks \cite{koshy2014analysis,biryukov}.
%Examples of these heuristics include \red{XYZ}.

\subsubsection{Diffusion}
In 2015, the Bitcoin reference implementation adopted a variant of these heuristics known as \emph{diffusion spreading} \cite{bitcoind}.
Under diffusion spreading, each node transmits or relays messages with independent, exponential delays to each neighbor on the P2P network.
In Bitcoin Core, the delays on outbound edges have twice the rate (i.e., half the expected delay) of inbound edges;
this is done to thwart supernode-based deanonymization attacks, since it is easier for malicious nodes to create inbound edges to honest nodes than force honest nodes to create outbound edges to the supernode \cite{bitcoind}.

Although diffusion closed some loopholes from trickle spreading, the decision to adopt it was not systematically motivated (as far as we know).
In fact, recent analysis suggests that trickle and diffusion fundamentally exhibit similar anonymity properties \cite{fanti2017}.
Hence, diffusion may not suffice as a standalone anonymity solution.
%However, the analysis and simulations in \cite{fanti2017} do not explicitly account for the rate asymmetry of diffusion in today's network.

%\begin{figure}[t]
%    \centering
%  \includegraphics[width=.4\textwidth]{figures/sym_vs_asym}
%  \caption{Probability of detection under symmetric diffusion and asymmetric diffusion of transactions.}
%  \label{fig:asymmetry}
%\end{figure}

%We demonstrate in Figure \ref{fig:asymmetry} that this asymmetry does not significantly improve the anonymity properties of diffusion. 
%Figure \ref{fig:asymmetry} plots the simulated probability of a group of supernodes correctly identifying a transaction source IP using the first-spy estimator on a 100-node graph constructed according to Algorithm \ref{algo:dreg_approx} (discussed in more detail in \S\ref{sec:model}).
%This probability is computed as a function of the number of supernodes, or equivalently, the number of connections a single supernode makes to each honest node.\footnote{In \cite{biryukov}, supernodes establish multiple connections to each honest node.}
%The red curve is computed using symmetric delays on inbound and outbound edges (i.e., exponential delays of the same rate); the blue curve uses the asymmetric delays of the real Bitcoin network.
%%We observe little overall difference between the two.
%While asymmetric diffusion does have a lower probability of detection, the difference is less than 15\% over most of the parameter space.
%This happens because the minimum of two independent exponential random variables of rate $\lambda$ is also an exponential random variable of rate $2\lambda$; 
%hence, a supernode can observe relayed transactions from a given node with the same delay distribution as if it were an outbound neighbor by establishing two inbound connections.
%Since supernodes are relatively easy and cheap to set up \cite{coinscope, biryukov}, such an attack is trivial.
%Therefore, asymmetric diffusion may not suffice as a standalone anonymity solution. %significantly deter deanonymization attacks.
%%This seems to happen because symmetric spreading schemes implicitly leak provenance metadata; 
%%while Bitcoin's diffusion implementation does introduce some asymmetry, it is not pronounced enough to provide significant anonymity benefits.

\subsubsection{Relaying through Tor}
Many privacy-conscious Bitcoin users connect to the Bitcoin network through Tor \cite{tor,biryukov2015bitcoin}.  
In principle, such users' transactions can, at best, be linked to a Tor exit node, assuming Tor provides sufficient anonymity. 
While this solution inherently breaks the symmetry of diffusion and is robust in many respects, there are some key drawbacks.
The first is that researchers have demonstrated eclipsing attacks on Bitcoin users who connect to the Bitcoin network through Tor \cite{biryukov2015bitcoin};
such attacks can be devastating from an anonymity perspective.
Even in the absence of eclipsing attacks, the approach requires users to be (a) aware of Bitcoin's P2P anonymity vulnerabilities, and (b) tech-savvy enough to connect to Bitcoin through Tor. 
Finally, this approach involves routing traffic through a third-party network that may be unwilling to support Bitcoin traffic on a large scale.
We ultimately seek scalable, in-network solutions that protect \emph{all} users rather than just the privacy-aware ones.


\subsubsection{Relaying through I2P}
Another option is to implement I2P over the underlying cryptocurrency P2P network \cite{i2p}.\footnote{I2P is an anonymity overlay designed to operate within P2P networks.} 
I2P provides similar unlinkability guarantees to Tor, and Monero \cite{monero} is currently integrating I2P into its peer-to-peer network.
%Like Tor, I2P would also break the symmetry of diffusion, thereby providing strong anonymity guarantees.
However, I2P is complex to implement; Monero has been developing this feature for at least three years \cite{kovri}, and the project is still in active development ~\cite{reddit_i2p}.
Given that Bitcoin has significant, well-documented anonymity weaknesses in its blockchain layer \cite{fistful}, the community may be unwilling to expend such  resources to patch anonymity vulnerabilities in the P2P layer.
Hence, simple, lightweight solutions are desirable.

\subsubsection{Dandelion} A recent paper proposed a two-phase, statistical approach to this problem called \Algo~ \cite{dand}. 
\Algo~ resembles Tor and I2P in the sense that transactions are forwarded along a randomly-selected line of nodes before being diffused. 
The key differences compared to Tor and I2P are: (a) \Algo~messages are unencrypted as they traverse the chain of nodes, and (b) different transactions from different nodes traverse the \emph{same} line; this (somewhat subtle) point leads to stronger anonymity guarantees than choosing independent lines for each transaction.
Indeed, \cite{dand} shows that \Algo~exhibits near-optimal anonymity guarantees, as measured by the adversary's ability to map transactions to their source IP addresses.
However, \Algo~ is presented in an idealized setting; 
adversarial parties are assumed to be honest-but-curious, and the paper does not address  practical deployment-related issues.
Indeed, we show that several of \cite{dand}'s anonymity claims are fragile to malicious nodes.

\subsubsection{Privacy-Aware Cryptocurrencies}
Finally, several projects have emerged that address the privacy vulnerabilities of Bitcoin's blockchain, including Monero \cite{monero}, Zcash \cite{sasson2014zerocash,miers2013zerocoin,zcash}, Tumblebit \cite{heilman2016tumblebit}, and Mimblewimble \cite{mimblewimble}.
While these papers are primarily motivated by blockchain vulnerabilities, some of them also address network vulnerabilities by asking users to adopt Tor \cite{heilman2016tumblebit} or incorporating network protections into the proposed cryptocurrency \cite{zcash,monero}.
We seek a solution that is inherently compatible with Bitcoin and independent of third-party networks like Tor. While our evaluation focuses on the Bitcoin network, our techniques are equally applicable to the other cryptocurrency networks, which use the same transaction propagation approach.

%\subsubsection{Summary}
%%Among the proposed solutions in this space, we contend that \Algo~ is the closest to a workable one: it is lightweight, distributed, and Bitcoin-compatible, while still providing some degree of provable, population-wide anonymity guarantees.
%In this paper, we propose a lightweight, provably-anonymous flooding policy that uses \Algo~ as a starting point.
%As discussed previously, \Algo~is far from practical in its current state.
%First and foremost, it is unclear if and how its anonymity guarantees extend to realistic attack scenarios with Byzantine nodes, partial deployment, etc.
%Indeed, we show that \Algo's anonymity guarantees are fragile to active attackers.
%Second, \cite{dand} did not actually evaluate the practical latency and/or implementation overhead of \Algo.
%In this paper, we address these weaknesses by proposing a revised policy, \Algopp, that provides stronger robustness and anonymity properties, both in theory and in practice.
%We also implement \Algopp~and test it in the Bitcoin network to demonstrate that it incurs minimal latency overhead compared to the status quo of diffusion-based broadcasting. 
%We begin by presenting a practical, lightweight attack and demonstrating its impact on the privacy guarantees of both diffusion and \Algo.  %adversarial model and problem formulation.

